Examining Racial Stereotypes in YouTube Autocomplete Suggestions

Autocomplete is a popular search feature that predicts queries based on user input and guides users to a set of potentially relevant suggestions. In this study, we examine what YouTube autocompletes suggest to users seeking information about race on the platform. Specifically, we perform an algorithm output audit of autocomplete suggestions for input queries about four racial groups and examine the stereotypes they embody. Using critical discourse analysis, we identify five major sociocultural contexts in which racial information appears -Appearance, Ability, Culture, Social Equity, and Manner. We found that the participatory nature of YouTube produces a multifaceted representation of race-related content in its search outputs, characterized by enduring historical biases, aggregated discrimination, and interracial tensions, while simultaneously depicting minority resistance and aspirations of a post-racial society. We call for innovations in content moderation policy design and enforcement to address existing racial harms in YouTube search outputs.

==> cut.tex <==
% ==== deleted content (0814~) ======

%%% Introduction

% This widespread deployment of the Autocomplete feature evinces a recognition that it can facilitate users' search process by navigating them to specific query selections and their corresponding content. 

% Recent research efforts have sought to expand our understanding of the influence of search autocomplete outputs beyond English-language Google search results. For example, these studies have explored a range of biases of these outputs in non-English languages \citep{chonka2023algorithmic}, non-Western-based platforms \citep{liu2024comparison}, and Google image results \citep{rogers2023algorithmic}. To recognize this importance and move this agenda further, this paper investigates racial bias in autocomplete outputs connected to YouTube video content that remains relatively unexplored. 

% Research methods + findings etc. (1p) broad level
%Thus, we analyzed racial bias in autocompletes with quantitative and qualitative approaches to understand the extent of racial disparity in this technology as well as the racial stereotypes reflected in autocompletes. Our study offers several contributions to prior literature on algorithmic biases. First, we reveal the prevalence of troubling biases in search autocompletes on the previously under-explored but vitally crucial platform, YouTube. Second, we qualitatively coded our data and engaged in a critical discourse analysis to examine the sociocultural effects of these biases. By considering the contexts within which such racially tinged autocomplete queries could be made and the user-uploaded content that may have shaped autocomplete results, we offer insights into how racial stereotypes may have been perpetuated and reinforced on the YouTube platform.
%Our findings can show the differences and similarities from the previous findings mainly from Google autocompletes. 

% Paper structure?
%This paper begins with a discussion of related work on racial stereotypes, algorithmic biases, and YouTube search autocomplete. Following this, we will discuss our research methods, including data collection and analysis procedures. Next, we will present our results and then conclude with a discussion of our core findings.





%%% Background and Related Work

%% Racial Stereotypes
\citep{us_census_multiracial_2021}

%% Asian
%These images characterized Asian men as depraved, lacking control, and weak \citep{said1977orientalism}. 
%(e.g., serving as cooks, waiters, and laundrymen)
%e.g., gowns, or serving as maids

%% Hispanic 
% Further, Hispanics are negatively stereotyped especially in the context of immigration, unlawful activity, and crime \citep{gonzalez2019stereotypical, dixon2015changing}. 


% Algorithmic Bias - concept added 

% Bias can be described as systematic and unfair discrimination of particular persons or groups emerging from computer systems \citep{friedman1996bias}. 

% When a systematic deviation in algorithmic outputs such as autocomplete is seen particularly in the form reflective of stereotypes and discrimination related to certain racial groups of people, we propose to call this \textit{racial bias} in our study.

% With the ever-increasing reliance on online systems for knowledge gain, algorithms that drive these systems have become increasingly important in shaping individuals' perceptions of the world around them \citep{gillespie2014relevance, kitchin2019thinking}. However, 

% With the ever-increasing reliance on online systems for knowledge gain, algorithms that drive these systems have become increasingly important in shaping individuals' perceptions of the world around them \citep{gillespie2014relevance, kitchin2019thinking}. Significant disparities in algorithmic outputs exist for certain social groups along the dimensions of gender, race, or religion \citep{abid2021persistent, kay2015unequal, sheng2019woman, sweeney2013discrimination}. 

% Notably, race is one of the salient attributes that trigger systematically biased outputs in technological systems. For example, Google ads indicative of arrest records were more noticeably responsive to the searches of Black-identifying first names than White-sounding names \citep{sweeney2013discrimination}. Such anecdotes suggest that algorithmic systems produce discriminatory outputs by race. As such, bias can be described as systematic and unfair discrimination of particular persons or groups emerging from computer systems \citep{friedman1996bias}. Discriminatory practices innate in algorithms called ``technological redlining" \citep[p.1]{noble2018algorithms} are likely found in the forms of reiterated misrepresentation or distortions against certain racial groups through Kay et al. approaches like ``stereotype exaggeration," ``systematic over-/under- representation," and ``qualitative differential representation." \citep{ferrara2023should, kay2015unequal, urman2024foreign}. In addition, from a quantitative perspective, exclusionary practices against racial minorities existing in traditional media tend to be repeatedly reflected in technology ecosystems such as facial algorithms \citep{grother2014face, klare2012face}. Therefore, our conceptualization of algorithmic bias is grounded in ``a systematic deviation from equality" implicitly assumed in algorithmic outputs \citep[p.8]{kordzadeh2022algorithmic}. As noted earlier, a systematic deviation may revolve around race. When a systematic deviation in algorithmic outcome is seen particularly in the form reflective of stereotypes and discrimination related to certain groups of people, we propose to call this racial bias in our study. 

% % Racial bias in Autocomplete
% Racial bias has been exhibited in suggestions created by automated systems \citep{al2020google, baker2013white, leidinger2023stereotypes, roy2020age}. For example, \citet{roy2020age} showed that Google search autocompletes contain age and gender stereotypes. They also found that as men and women become older, men are depicted as being in a position of gaining power whereas women are described as having a loss of visual appeal. Focusing on more diverse identity groups, Baker and Potts found that the autocomplete feature of the Google search engine produces more predictions with negative stereotypes for Black, gay, and male groups than other groups \citep{baker2013white}. Besides Google, autocompletes from another general-purpose search engine, Yahoo, include a large number of negative stereotypes for Latinos, such as stupid or loud \citep{leidinger2023stereotypes}. In sum, the evidence from these aforementioned studies suggests that autocompletes expose end-users to information or content with biased and stereotyping perspectives toward certain groups. 

% % Negative impact of racial bias arising from autocomplete + Research Questions
% In this respect, researchers have shown concerns about the potential risks of autocomplete function in eliciting and reinforcing discriminatory and stereotypical perceptions about certain social groups \citep{leidinger2023stereotypes, rogers2023algorithmic}. Algorithmic outputs built on human language analysis may partly reflect existing biases or stereotypic attributes latent in society \citep{ferrara2023should}. Yet, the true challenge of algorithmic bias may arise when we take an uncritical approach to those outputs \citep{shugars2024critical}. We should recognize clearly that systematically discriminatory outputs against certain racial groups, such as rampant pornographic images of black girls in Google, are fundamental to technological systems rather than simply a glitch \citep{noble2018algorithms}, and it is crucial that we recognize such discriminations when they manifest. We therefore ask the following research question in this article: 
% \begin{quote}
%     \textbf{\textit{Do YouTube autocomplete suggestions reflect racial bias?}}
% \end{quote}

% % quantitative and qualitative
% To answer this question, we conducted an algorithm audit of YouTube autocomplete outputs. From a quantitative perspective, we compared the numbers of autocompletes as well as the input queries with autocompletes generated by race to examine to what extent each racial group is included or excluded in the automated systems. In addition to the visibility of the racial groups, we examined how the depiction of each racial group is qualitatively different in autocomplete, with a focus on surfacing stereotypes. We therefore collected YouTube autocomplete results for race-related input search queries and analyzed them. We next describe the details of our method below.


%%% Method

%% Data collection 
%For example, the combined forms were ``Is a White person...?," ``Black women should...," ``Asian man can...,'' and ``Do Hispanic people...?.''

% July 27, 2023 and August 14, 2023 
% the effect of personalization \citep{juneja2023assessing} and prior browsing history \citep{hussein2020measuring}.

% In sum, we collected YouTube autocompletes from the five states three times. 

%% Data Preparation
% To get a comprehensive understanding of YouTube autocomplete suggestions in the U.S., 

% The dataset consists of a total of 459 autocomplete results. 

%(White: 205, Black: 184, Asian: 50, and Hispanic: 20, respectively). 
% \begin{table*}[b]
%   \caption{The Descriptive Statistics of Final Dataset}
%   \label{tab:stats}
%   \centering
%   \begin{tabular}{cccc}
%     \toprule
%     Category & \# Autocompletes & \# Generative input queries & Avg. autocompletes per input query \\
%     \midrule
%         White & 102 & 33& 3.091\\
%         Black & 96 & 31& 3.097\\
%         Asian & 38 & 16& 2.375\\
%         Hispanic & 10 & 7 & 1.428\\
%         \hline
%         Total & 246 & 87& -\\
%     \bottomrule
%   \end{tabular}
% \end{table*}

%% Data Analysis

% Content analysis
% The qualitative content analysis was conducted for data analysis. This method is an inductive approach to content analysis, which is a method largely used in analyzing data in written, verbal, or visual forms to attain concepts or categories that describe the phenomenon .  
% This approach is particularly known to be useful when the previous knowledge about the phenomenon is not enough or fragmented \citep{elo2008qualitative}. Thus, inductive content analysis is appropriate for our research given the lack of former knowledge on this topic. In addition, 
% Thus, this study conducts qualitative content analysis given its methodological strength for the goal of our study, investigating the racial biases in YouTube autocomplete.
% presents the results of the categorization scheme for the racial groups. 
% \newline 



%%% Results

%% Quantitative Analusis
% This means about 91\% of the input queries didn't generate the autocompletion regarding Hispanic groups. 

%% Qualitative Analysis
% Some autocomplete was produced in the form of incomplete sentences or included grammatical errors in its output (e.g., ``Can a white guy won [sic] an Asian beauty pageant?). We analyzed each autocomplete verbatim as it was originally generated. We also present the original form of the autocomplete when we provide the corresponding examples in the result section. 

%% Beauty
%% Facial Hair
% This reflects the feminized stereotype of Asian men in the U.S. \citep{chen1996feminization}. 
% \citep{neave2008effects}
%Men with a beard or facial hair have been perceived as more attractive, masculine, and dominant compared to those without a beard \citep{neave2008effects}. 

%% Capability
%% Talent
% \citep{biernat1994shifting}.
% For example, there were positive autocompletes (``White girl can rap,'' ``White girl can sing") and negative autocompletes (``White boys can't dance,'' ``White people can't dance''). 
% are a reflection of stereotypical awareness of Whites, possibly leading the public to strengthen the image of an inferior White athlete in physical performance. 

% Financial
% the stereotype that the poor are mostly Blacks in the United States. 
% portrayed the poor as substantially more black than in really the case
% This aligns with prior research findings and past results that the poor are portrayed as Blacks in the media more than their true cases 
% They treat the Black woman unfairly, refusing her to try the dress on and increasing the price of the dress because they think she can't afford the dress. However, the woman is an innocent customer who can afford it. 

%% Intellectual 
% \citep{lee2008th}
% These results also show that autocomplete reflects the opposite stereotypes for the intelligence of Asians and Blacks. 
% This seemingly positive stereotype can be harmful and misleading in that it can hide the diversity among Asians, cause interracial tension, and discourage Asians from revealing problems and seeking assistance \cite{lee2008th}. - move 

%% Culture
%% Cultural Heritage
% First, we found that Whites, Blacks, and Asians had autocompletes that were associated with cultural practices. Those autocomplete suggestions showed the multiple acts of cultural appropriation, but the context in which cultural appropriation occurs was different based on asymmetrical power relations between racial groups. Primarily, the text elicited by autocompletes reflected the directionality of a dominant group toward the culture of a minority group. For example, the autocompletes related to White groups revealed an implicit act of consumption of indigenous Black cultures with no understanding of or respect for its native contexts (e.g., ``White girl can dance African''). Some autocompletes show the participation of White people in the exploitation of a particular heritage from Asian culture, thereby reflecting the forms of cultural appropriation by members of White groups across Asian and Black cultures (``Can a white guy won an Asian beauty pageant?,'' ``Can a white guy make a kpop group?''). In contrast, the keyword `Black' elicited an autocomplete related to the use of Asian cultural elements, which was only one result (``Can a Black person become a kpop idol?'').
% Similarly, a tendency for appropriation of the properties of Asian cultures by  White groups was reflected in autocompletes related to garments. A kimono is Japan's traditional clothing that is derived from Japanese culture. The trend to appropriate such garments of Eastern culture was shown in the autocompletes for White groups (``Can a White person wear a kimono?''). Contrary to this, autocompletes for the Asian group did not produce any relevant results though the kimono is a symbol of Asian culture. 
% The autocomplete result shows the acts of Whites to appropriate blackness inherently through replications of physical appearance \citep{cherid2021ain}.
% In a few cases, autocompletes in this category directed users to videos depicting the harms of cultural appropriation. 
% reflect the unidirectionality of exchange between different cultures. It was sometimes the case that the aforementioned autocomplete suggestions guided users to a list of video content with diverse voices and perspectives on cultural appropriation, particularly the acts driven by Whites. However, given that YouTube autocomplete failed to directly elicit diverse perspectives in their text generation itself, we confirm that there exist potential asymmetries between racial groups in the suggestion of YouTube's autocomplete regarding the perspective of cultural appropriation. 
% compared to other racial groups. 
% Most of the autocomplete for Asians was associated with the video content created by an Asian YouTuber Steven He, who has 12.3 million subscribers.\footnote{https://www.youtube.com/@StevenHe} His YouTube content usually had a fictional Asian character, often portrayed as a dad, with an ``Asian'' accent and having expectations that Asians should be good at math, hard-working, and pursuing high economic and academic goals. 
% The videos for other autocompletes also reflect similar stereotypical images of Asians (``when an Asian is kidnapped,'' ``when an Asian is president,'' ``when an Asian is your substitute,'' etc.). 
% The shared characteristics of the resulting videos are that they reinforce the differences and the stereotypical image of Asians. 
%negative stereotypes about them.
%This term embodies positive characteristics like agency, sexuality, beauty, and boldness but also negative attributes like aggression and violence \citep{wu2023study}. 
% at the intersection of cultural practices and race 
% were also not associated with cultural appropriation, but curiously, they


%% Lifestyle
% Notably, the representation of a typical White female tends to be associated with negative stereotypes. 

%% Language
% These can be seen as a reflection of the act of social categorization between self and others through how a person speaks within a multicultural society. 
% In our analysis, we found that all racial groups had autocomplete results associated with language. 
% The autocompletes related to language were broadly divided into the forms of two verbal communication: voices and accents. 

%% Relationships
%and ``These Asian Girls Do Not Like Asian Men?!.'


%% Social Issues
%% Diversity/Inclusion
% As seen from recent statistics, there is still ongoing inequality against underrepresented groups such as Blacks or Hispanics in the industry. Autocompletes seem to reflect the more diverse and inclusive pursuits of other minorities in the casting process. YouTube autocompletes in this category reveal frustrations about inequalities in the racial representation of character portrayals on the screen, thereby contributing to promoting an incremental change in casting decisions in the industry.

% Racial Justice 
%brooks2020using, 
% that contributed to the rise of the `Black Lives Matter' movement \citep{clayton2018black}.
% \newline 
% First, there existed an autocomplete result related to drama lines satirizing critically White privilege (``That is a white man's luxury''). The text of autocomplete suggestions was a part of the following lines of the character ‘Stan Edgar’ in the drama named `The Boys': ``I can’t lash out like some raging entitled maniac. That is a white man's luxury.'' Indeed, we confirm that the autocomplete guided users to a list of the corresponding drama content. The lines mentioned by the African-American character of the drama may convey that expressing feelings and acting with no restrictions in society mirrors the White privilege itself. These autocomplete results seem to reveal uneven societal expectations and constraints toward other racial groups that are rarely emphasized on White racial groups. 
% Meanwhile, some autocomplete included the messages of social movements in which White racial groups were placed at the center.
% Our findings may confirm that there is lacking attention to a balanced reflection of voices and perspectives from different social movements by overlooking including the messages of `Black Lives Matter' directly in autocomplete itself. 

%% Traits
%% Lazy/Inappropriate
% The distorted perceptions of Blacks as lazy have also been associated with the stereotypes of their financial capacity \citep{gilens1996race}, as described above. 
% These shorts often start Black people criticizing this stereotype but soon realizing that their smoke alarm is chirping. 



%%% Discussion

% More troublingly, end-users may perceive site-generated snippets like search autosuggestions as more reliable than other user-generated content posted on these sites \citep{muller2021ethics}.

% The common key characteristic across various interventions is `autonomy' that is delegated to AI agents on behalf of human communicators \citep{hancock2020ai}. 

% As independent researchers, we do not have visibility into the granular details of how users engage with AI-based snippets like search autocompletes.

%% Ethical Deployment of AI-Generated Suggestions

% Autocomplete
% could cause problems since the end-users might accept the content that contains stereotypical viewpoints without critical perspective due to the trust on the digital platforms and the AI-based tools. 
% Thus, it is vital that platforms perform a regular, careful audit process of AI-generated outcomes. 
% Our analysis shows the difficulties in identifying stereotypical content due to the complex nature of video-sharing platforms. For example, we found autocompletes that show explicit racial stereotypes such as ``Black women can't buy a dress.'' Our results showed that it is hard to determine this is problematic autocomplete because its resulting video contains critical viewpoints and aims to break negative stereotypes. Similarly, while the slogan ‘White Lives Matter’ is directly contained in the text of autocomplete suggestions, the corresponding lists of the videos include diverse voices and views including criticism of the movement ‘White Lives Matter’. Thus, determining the stereotypical content solely based on the autocomplete could be misleading. Due to the nature of YouTube, automating content moderation for identifying stereotypical autocomplete is challenging. This suggests the need for human moderators who can understand the subtle nuances, contexts, and purpose of the videos. 

% LLM
% We also contend that it is important to assess how people perceive such autogenerated content where they are divorced from the context in which they were first inputted. 

% (Qual results added)
% there was lacking evidence about the opposite flow to be taken by members of Black or Asian cultures toward White culture. 


% Contributions
% Lastly, we used CDA for in-depth analysis to reflect the power dynamics in racial groups in the U.S.




-- Discussion original content (0821)-----

% \subsection{Ethical Deployment of AI-Generated Suggestions}
% % autocomplete - bias/ethical issue
% Today, almost all major digital platforms deploy AI-based tools to generate a variety of information snippets. These tools are usually trained on user-uploaded data and built with prediction algorithms that incorporate a range of factors relevant to the task at hand. However, our results from this study suggest that such AI-based tools do not fully take into account how their outputs could be racially insensitive. More troublingly, end-users may perceive site-generated snippets like search autosuggestions as more reliable than other user-generated content posted on these sites \citep{muller2021ethics}. This raises the likelihood that some users, especially those who largely trust digital platforms and their tools, are influenced by the stereotypical viewpoints embedded within such AI-generated outputs without critically considering that they may be biased. 

% % future ver of autocomplete - llm 
% This has implications for the increasing use of LLM-based outputs for a wide range of user-facing interfaces. For example, beyond search autocompletes, AI mediation has been applied to enable features such as auto-corrections and auto-responses. The common key characteristic across various interventions is `autonomy' that is delegated to AI agents on behalf of human communicators \citep{hancock2020ai}. Given that AI agents are increasingly likely to secure a significant amount of autonomy in future tasks, the biases embedded in AI agents may be still a potential challenge. \citet{williams2024bias} found a critical nudge effect of autocomplete suggestions, showing that participants shifted their attitudes along with AI-biased suggestions and had even no awareness of AI bias and impacts. As prior research shows \citep {chancellor2019taxonomy}, the black-box nature of such AI-based technologies precludes users from understanding how their outputs were generated, and especially, how they could embed identity-based biases. These results align with our concern that biased algorithmic outputs may adversely influence users’ perceptions and attitudes against certain social groups. 

% % moderation strategy - platform how? 
% Given the extent to which people rely on digital technologies, especially search engines, to get information and develop informed viewpoints on any given topic, it is critical that such technologies invest in mitigating discriminatory and stereotypical outputs against specific racial groups. To achieve this, we recommend that content curation infrastructures incorporate a regular review of automatically generated texts and suggested content, at least for the most frequently searched, culturally-sensitive topics. 

% Our analysis shows that in some cases (e.g., ``Black women can't buy a dress,'' ``White Lives Matter''), the autocomplete suggestions themselves were problematic but many resulting videos offered a more nuanced understanding and in some cases, even break pre-existing racial stereotypes. This suggests that human moderators who can understand the subtle nuances, contexts, and purpose of the videos could be deployed to help shape such algorithmic outputs. As independent researchers, we do not have visibility into the granular details of how users engage with AI-based snippets like search autocomplete. Future work can build upon this research by examining the details of how these features epistemically influence end-users, e.g., it would be informative to analyze the relative influence of search autocomplete texts and their resulting videos. 

% \subsection{The State of Race in the US Today}
% While popular narratives often proclaim that we live in a post-race society, the sheer number and diversity of racially biased autocomplete suggestions we found in our analyses reflect that this is not the case. 

% % (Quan results added)
% Our study suggests that racial stereotypes keep being generated and perpetuated on digital platforms through their autocomplete features despite a range of efforts to reduce racial discrimination in many offline settings. 

% % First, we identified that autocompletes related to White and Black are more frequently recommended compared to Asian and Hispanic. This finding suggests the main technical feature on YouTube under-represent the specific racial groups who are often recognized as minorities in U.S. society. Our findings also show the systematic over and under-representation of racial groups \citep{kay2015unequal} on YouTube and replicate the under-representations of Latinos and Asians in the mainstream media from previous research \citep{stamps2019really}. 

% % (Qual results added)
% Our analysis shows the continued sustenance of negative racial stereotypes that persist to this day. We especially found troubling stereotypes regarding the following aspects: Whites' position in the context of cultural appropriation, Blacks with negative characteristics (e.g., laziness, dirt, etc), Asians as the model minority or forever foreigners, and Hispanics as the peripheral characters in the entertainment industry. Our analysis highlights systematic differences in stereotypical representation of different racial groups. In addition, we found evidence of systematic under- or over-representation across racial groups. For example, while Black viewpoints such as ‘Black Lives Matter’ were omitted, white voices were directly represented in the text suggestions of autocomplete itself. Besides, autocompletes included the White group's diverse appropriative acts of other cultures’ traditional practices. This shows that YouTube autocomplete suggestions tend to reflect no substantive reciprocity between White and non-White cultures. Hence, our results reveal asymmetries across racial groups in the suggestion of YouTube’s autocomplete. We contend that there exists a reflection of the imbalanced power relations between racial groups in YouTube's algorithmic systems.

% Our analysis shows that YouTube autocomplete goes beyond the binary focus on White versus Black races and instead suggests a more complex cultural milieu that seeks to characterize, often negatively, other races, such as Asians and Hispanics as well. The U.S. is a multi-racial/ethnic society as well as a country with 238 million YouTube users \citep{statista_youtube_users}. Exposing stereotypical autocomplete about others or even their own racial groups could potentially reinforce the distorted perspectives toward specific racial groups. Given the popularity of YouTube, this could lead to detrimental impacts, such as inducing harmful assumptions about a specific race to future generations or naive users who have neutral perspectives.

% In addition, the formats of YouTube videos around stereotypical autocomplete give insight into how stereotypes are perpetuated and even recommended in digital platforms. We confirmed that stereotypical portrayals against certain racial groups in existing mainstream media content are readily reproduced and amplified on YouTube. For example, some autocomplete directly generates the existing title (e.g., ``White Men Can't Jump'' ) or lines (e.g., ``That is a white man's luxury'') from mainstream popular culture, thereby directing users to the lists of the corresponding media content with the stereotypical attributes. As such, autocomplete suggestions contribute to promoting the delivery of distorted racial images already being depicted in popular media. Our analysis also found that racial stereotypes are delivered in the form of \textit{ethnic humor} and memes. In our study, we found that an Asian YouTube creator gained fame and success by creating multiple videos exploiting Asian stereotypes. Such content is presumably perceived as funny and enjoyable by YouTube users, as evidenced by the millions of views it generates. Additionally, we found that stereotypes are conveyed as a joke and a new play culture in a short-form YouTube video (e.g., ``Black people can't hear smoke detectors''). This suggests that racial stereotypes are often delivered as a fun joke and memes on digital platforms, which makes it hard to identify this content as potentially harmful and dangerous. Overall, this suggests that as a country and culture, we have a long way to go in achieving racial harmony and resisting the otherization of racial minorities.

% Our study shows how digital platforms can be leveraged as a lens to understand the current state of race relationships. Identifying racial stereotypes through such means can offer a way to examine the present challenges and shape literacy measures that counter those stereotypes. We need a transformative approach to systematically counter these stereotypes, both online and offline. Thus, content moderation and AI audit efforts need to be paired with broader educational, cultural and policy initiatives to combat racial biases.

% % \subsection{Contributions}
% % This study examines racial biases in autocomplete suggestions on YouTube, a global video-sharing platform. Our study contributes to prior literature which largely focused on studying how search engines autocompletes incorporate biases \citep{leidinger2023stereotypes, roy2020age}. Our results show how the four racial groups are described differently in autocompletes. We found the similar findings from the previous research and the distinctive findings as well. For example, \citet{leidinger2023stereotypes} found that Yahoo has autocompletes about Black people that include terms like aggressive, violent, and angry, which are also found in our study. Our results, however, also found that Black people are associated with laziness and lack of financial ability in YouTube autocomplete that are not appeared in the previous research. Likewise, this research shows the perpetuating racial stereotypes surrounding online platforms as well as the new descriptions for racial groups on YouTube. In addition, we analyzed the autocomplete in-depth by viewing its resulting video to understand its latent meaning as well as the manifest meaning of autocomplete. This approach could help us capture the contexts of the autocomplete and enable us to analyze the autocomplete deeper than surface level. 

% % \subsection{Limitations and Future Work}
% Intersectional attributes just beyond single social identities may sometimes act as the basic category of the individual perception process, possibly activating distinct stereotypes on intersecting social groups \citep{goff2008ain}. Indeed, compared to White women, the intersectional identity of Black women or Latina women included a higher degree of unique stereotypic attributes not typically associated with a collection of every single identity such as gender or ethnicity \citep{ghavami2013intersectional}. 
